Scene Informer: Anchor-based Occlusion Inference and Trajectory Prediction in Partially Observable Environments

Navigating complex and dynamic environments requires autonomous vehicles (AVs) to reason about both visible and occluded regions. This involves predicting the future motion of observed agents, inferring occluded ones, and modeling their interactions based on vectorized scene representations of the partially observable environment. However, prior work on occlusion inference and trajectory prediction have developed in isolation, with the former based on simplified rasterized methods and the latter assuming full environment observability. We introduce the Scene Informer, a unified approach for predicting both observed agent trajectories and inferring occlusions in a partially observable setting. It uses a transformer to aggregate various input modalities and facilitate selective queries on occlusions that might intersect with the AV's planned path. The framework estimates occupancy probabilities and likely trajectories for occlusions, as well as forecast motion for observed agents. We explore common observability assumptions in both domains and their performance impact. Our approach outperforms existing methods in both occupancy prediction and trajectory prediction in partially observable setting on the Waymo Open Motion Dataset.

==> figures/figures/ablation.tex <==
\renewcommand{\thesubfigure}{}
\begin{figure*}[ht]
\tiny
\centering
\subfigure[Scene 1: Trajectories]{\label{fig:a}\includegraphics[width=36mm]{new_figures/Modified_Ablation_4.pdf}}
\hspace{1cm} % adjust this value to change horizontal spacing
\subfigure[Scene 1: Occupancy]{\label{fig:b}\includegraphics[width=36mm]{new_figures/Modified_Ablation_1.pdf}}
\hspace{1cm} % adjust this value to change horizontal spacing
\subfigure[Scene 2: Trajectories]{\label{fig:a}\includegraphics[width=36mm]{new_figures/Modified_Ablation_3.pdf}}
\hspace{1cm} % adjust this value to change horizontal spacing
\subfigure[Scene 2: Occupancy]{\label{fig:b}\includegraphics[width=36mm]{new_figures/Modified_Ablation_2.pdf}}
\vspace{-0.25cm} % adjust this value to change vertical spacing between rows
\caption{Impact of observed agents' histories on the occlusion inference performance. We modify the observed trajectories of two agents (\bluecircle and \greentriangle). In Scene 1, we visualize a scenario where a \greentriangle\ is stationary and a \bluecircle\ is moving forward. For an anchor \redanchor, our approach predicts occupancy with low probability and vertical motion from the top to the bottom of the intersection. In Scene 2, we visualize the predictions for a modified scenario. The \greentriangle\ is approaching quickly the intersection and the \bluecircle\ is stationary. Scene Informer realistically adapts its occupancy and trajectory predictions based on the observed motion of other agents. It is now highly likely that the anchor in the middle of the occlusion is occupied, and a majority of predicted trajectories are horizontal from the left to right of the intersection.}
\vspace{-0.3cm}
  \label{fig:ablation}
 \end{figure*}
\renewcommand{\thesubfigure}{\alph{subfigure})}
%blue_circle = orange circle

==> figures/figures/numerical_results.tex <==
% \begin{table*}[h]
%     \caption{Comparison of different variations of Occlusion Informer and baselines. Occlusion Informer with full observability and auxiliary task outperforms all baselines on classification metrics. Occlusion Informer with Transformer encoder \& decoder pairing excels and the trajectory prediction.}
%       \begin{center}
%         \begin{tabular}{@{}llllrrrrrr@{}} \toprule
%         \multicolumn{2}{c}{Method} & &  & Acc $(\uparrow)$  & Free Acc  $(\uparrow)$ & Occ Acc $(\uparrow)$  & minFDE $(\downarrow)$ & minADE $(\downarrow)$ \\ \midrule
%         \multicolumn{2}{l}{Occlusion Informer (ours)}  \\ 
%         Encoder & Decoder & Full Obs. & Aux. \\ \midrule
%         Transformer & Transformer & \checkmark & \checkmark & 0.745 & 0.746 & 0.709 & \textbf{0.201} & \textbf{0.094} \\ 
%         Transformer & Transformer & \checkmark & & 0.805 & \textbf{0.816} & 0.556 & 1.841 & 0.815 \\
%         Transformer & MLP & \checkmark & \checkmark & 0.614 & 0.612 & \textbf{0.721} & 0.406 & 0.180  \\
%         Transformer & MLP & \checkmark &  & 0.778 & 0.783 & 0.486 & 2.158 & 0.983   \\ 
%         MLP & MLP & \checkmark & \checkmark  & 0.614  & 0.614 & 0.621 & 0.949 & 0.388  \\
%         MLP & MLP & \checkmark & & \textbf{0.818} & \textbf{0.828} & 0.434 & 1.426  & 1.071  \\ \midrule
%         Transformer & Transformer & &   \checkmark & 0.686 & 0.686 & 0.723 & \textbf{0.489} & \textbf{0.234}  \\
%         Transformer & Transformer & &  & 0.802  & 0.806 & 0.566 & 1.867 & 0.975  \\ 
%         Transformer & MLP &  & \checkmark & 0.466 & 0.459 & 0.831 & 0.933 & 0.466 \\
%         Transformer & MLP &  & & \textbf{0.826} & \textbf{0.832} & 0.472 & 1.361 & 0.663   \\
%         MLP & MLP &  & \checkmark  & 0.637 & 0.638 & 0.615 & 1.452 & 0.691 \\
%         MLP & MLP & & & 0.359 & 0.350 & \textbf{0.885} & 1.798 & 0.998 \\ \midrule  
%         K-means PaS \citep{afolabi2018people} &  & \checkmark & N/A & 0.614 & 0.613 & 0.664  & N/A & N/A \\
%         GMM PaS \citep{itkinaicra2022}  &  & \checkmark & N/A & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
%         \end{tabular}
%         \label{table:results}
%         \end{center}
% \end{table*} 


\begin{table*}[h]
    \caption{Comparison of different variations of Occlusion Informer and baselines. Occlusion Informer with full observability and auxiliary task outperforms all baselines on classification metrics. Occlusion Informer with Transformer encoder \& decoder pairing excels and the trajectory prediction.}
      \begin{center}
        \begin{tabular}{@{}llllrrrrrr@{}} \toprule
        Model & Full Obs. & Acc $(\uparrow)$  & Free Acc  $(\uparrow)$ & Occ Acc $(\uparrow)$  & minFDE $(\downarrow)$ & minADE $(\downarrow)$ \\ \midrule
        K-means PaS~\cite{afolabi2018people} & \checkmark & 0.614 & 0.613 & 0.664  & N/A & N/A \\
        GMM PaS~\cite{itkinaicra2022} & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\
        MAVOI~\cite{itkinaicra2022} & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
        Scene Informer (ours) & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
        Scene Informer (ours) & & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
        \end{tabular}
        %\label{table:results}
        \end{center}
\end{table*} 

% \begin{table*}[h]
%     \caption{Comparison of different variations of Occlusion Informer and baselines. Occlusion Informer with full observability and auxiliary task outperforms all baselines on classification metrics. Occlusion Informer with Transformer encoder \& decoder pairing excels and the trajectory prediction.}
%       \begin{center}
%         \begin{tabular}{@{}lllrrrrrr@{}} \toprule
%         \multicolumn{2}{c}{Method}  & \multicolumn{3}{c}{Trajectory Prediction} & \multicolumn{2}{c}{Occlusion Inference} \\ \midrule
%         Model & Full Obs.  & Full  & 0.5 & Lim. & minFDE $(\downarrow)$ & minADE $(\downarrow)$  \\ \midrule 
%         K-means PaS~\cite{afolabi2018people}  & \checkmark  & 0.614 & 0.613 & 0.664  & N/A & N/A \\
%         GMM PaS~\cite{itkinaicra2022}  & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\
%         MAVOI~\cite{itkinaicra2022}  & \checkmark  & 0.614 & 0.613 & 0.664  & N/A & N/A \\\midrule
%         \end{tabular}
%         \label{table:results_v2}
%         \end{center}
% \end{table*} 


==> figures/figures/prediction.tex <==
\begin{figure*}[ht]
\tiny
\centering     %%% not \center
\subfigure[Scene 1: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_3_b-2_False_False.pdf}}
\subfigure[Scene 1: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_3_b-2_False_False.pdf}}
\subfigure[Scene 2: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_47_b-3_False_False.pdf}}
\subfigure[Scene 2: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_47_b-3_False_False.pdf}}

\subfigure[Scene 3: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_289_b-0_False_False.pdf}}
\subfigure[Scene 3: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_289_b-0_False_False.pdf}}
\subfigure[Scene 4: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_291_b-0_False_False.pdf}}
\subfigure[Scene 4: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_291_b-0_False_False.pdf}}

\caption{Scene Informer prediction. We predict both occluded and observed objects represented as black dots. Dotted blue and green lines indicate observation, and ground truth future trajectories, respectively. Anchors are located inside the occlusion polygon (grey) from the perspective of the ego-vehicle (yellow star). Their intensity represents the probability of occupancy. For all scenarios, our approach predicts a high probability of occupancy for the ground truth occluded objects and outputs realistic future trajectories.}
\vspace{-0.3cm}
\label{fig:results}
\end{figure*}


==> figures/figures/visbility.tex <==
% \begin{figure}[h]
% \label{fig:dataset}
% \centering     %%% not \center
% \subfigure[Full]{\label{fig:a}\includegraphics[width=25mm]{figures/full_vis.png}}
% \subfigure[Limited]{\label{fig:b}\includegraphics[width=25mm]{figures/limit_vis.png}}
% \caption{Visualization of the occlusion inference dataset. (Left) Full observability dataset (Right) Limited observability with missing occluded objects from the perspective of the ego-vehicle. Past trajectories and future trajectories are visualized with blue and green colors, respectively. Each data sample contains only single occlusion (grey polygon) from the perspective of the ego vehicle (star). Red dots are anchors which are provided to the decoder. During optimization, we are matching the closest anchor to the to-be-inferred future trajectory.}
% \vspace{-0.3cm}
% \label{fig:dataset}
% \end{figure}

\begin{figure}[ht]
\tiny
\centering     %%% not \center
\subfigure[Full Obs]{\label{fig:a}\includegraphics[width=33mm]{new_figures/2_244_True_567-True_0.35_False_b_0_False_False_v2.pdf}}
\subfigure[Partial Obs (\SI{50}{\percent})]{\label{fig:a}\includegraphics[width=33mm]{new_figures/full_obs.pdf}}
\subfigure[Limited Obs]{\label{fig:b}\includegraphics[width=33mm]{new_figures/limited_obs.pdf}}
\subfigure[Full Obs (Occ. Inf.)]{\label{fig:b}\includegraphics[width=33mm]{new_figures/full_obs.pdf}}
% \subfigure[Scene 3: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_289_b-0_False_False.pdf}}
% \subfigure[Scene 3: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_289_b-0_False_False.pdf}}
% \subfigure[Scene 4: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_291_b-0_False_False.pdf}}
% \subfigure[Scene 4: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_291_b-0_False_False.pdf}}

\caption{Visualization of the occlusion inference dataset. (Left) Full observability dataset (Right) Limited observability with missing occluded objects from the perspective of the ego-vehicle. Past trajectories and future trajectories are visualized with blue and green colors, respectively. Each data sample contains only single occlusion (grey polygon) from the perspective of the ego vehicle (star). Red dots are anchors which are provided to the decoder. During optimization, we are matching the closest anchor to the to-be-inferred future trajectory.}
\vspace{-0.3cm}
\label{fig:results}
\end{figure}


==> figures/numerical_results.tex <==
% \begin{table*}[h]
%     \caption{Comparison of different variations of Occlusion Informer and baselines. Occlusion Informer with full observability and auxiliary task outperforms all baselines on classification metrics. Occlusion Informer with Transformer encoder \& decoder pairing excels and the trajectory prediction.}
%       \begin{center}
%         \begin{tabular}{@{}llllrrrrrr@{}} \toprule
%         \multicolumn{2}{c}{Method} & &  & Acc $(\uparrow)$  & Free Acc  $(\uparrow)$ & Occ Acc $(\uparrow)$  & minFDE $(\downarrow)$ & minADE $(\downarrow)$ \\ \midrule
%         \multicolumn{2}{l}{Occlusion Informer (ours)}  \\ 
%         Encoder & Decoder & Full Obs. & Aux. \\ \midrule
%         Transformer & Transformer & \checkmark & \checkmark & 0.745 & 0.746 & 0.709 & \textbf{0.201} & \textbf{0.094} \\ 
%         Transformer & Transformer & \checkmark & & 0.805 & \textbf{0.816} & 0.556 & 1.841 & 0.815 \\
%         Transformer & MLP & \checkmark & \checkmark & 0.614 & 0.612 & \textbf{0.721} & 0.406 & 0.180  \\
%         Transformer & MLP & \checkmark &  & 0.778 & 0.783 & 0.486 & 2.158 & 0.983   \\ 
%         MLP & MLP & \checkmark & \checkmark  & 0.614  & 0.614 & 0.621 & 0.949 & 0.388  \\
%         MLP & MLP & \checkmark & & \textbf{0.818} & \textbf{0.828} & 0.434 & 1.426  & 1.071  \\ \midrule
%         Transformer & Transformer & &   \checkmark & 0.686 & 0.686 & 0.723 & \textbf{0.489} & \textbf{0.234}  \\
%         Transformer & Transformer & &  & 0.802  & 0.806 & 0.566 & 1.867 & 0.975  \\ 
%         Transformer & MLP &  & \checkmark & 0.466 & 0.459 & 0.831 & 0.933 & 0.466 \\
%         Transformer & MLP &  & & \textbf{0.826} & \textbf{0.832} & 0.472 & 1.361 & 0.663   \\
%         MLP & MLP &  & \checkmark  & 0.637 & 0.638 & 0.615 & 1.452 & 0.691 \\
%         MLP & MLP & & & 0.359 & 0.350 & \textbf{0.885} & 1.798 & 0.998 \\ \midrule  
%         K-means PaS \citep{afolabi2018people} &  & \checkmark & N/A & 0.614 & 0.613 & 0.664  & N/A & N/A \\
%         GMM PaS \citep{itkinaicra2022}  &  & \checkmark & N/A & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
%         \end{tabular}
%         \label{table:results}
%         \end{center}
% \end{table*} 


\begin{table*}[h]
    \caption{Comparison of different variations of Occlusion Informer and baselines. Occlusion Informer with full observability and auxiliary task outperforms all baselines on classification metrics. Occlusion Informer with Transformer encoder \& decoder pairing excels and the trajectory prediction.}
      \begin{center}
        \begin{tabular}{@{}llllrrrrrr@{}} \toprule
        Model & Full Obs. & Acc $(\uparrow)$  & Free Acc  $(\uparrow)$ & Occ Acc $(\uparrow)$  & minFDE $(\downarrow)$ & minADE $(\downarrow)$ \\ \midrule
        K-means PaS~\cite{afolabi2018people} & \checkmark & 0.614 & 0.613 & 0.664  & N/A & N/A \\
        GMM PaS~\cite{itkinaicra2022} & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\
        MAVOI~\cite{itkinaicra2022} & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
        Scene Informer (ours) & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
        Scene Informer (ours) & & 0.536 & 0.532 & 0.685 & N/A & N/A \\ \midrule
        \end{tabular}
        %\label{table:results}
        \end{center}
\end{table*} 

% \begin{table*}[h]
%     \caption{Comparison of different variations of Occlusion Informer and baselines. Occlusion Informer with full observability and auxiliary task outperforms all baselines on classification metrics. Occlusion Informer with Transformer encoder \& decoder pairing excels and the trajectory prediction.}
%       \begin{center}
%         \begin{tabular}{@{}lllrrrrrr@{}} \toprule
%         \multicolumn{2}{c}{Method}  & \multicolumn{3}{c}{Trajectory Prediction} & \multicolumn{2}{c}{Occlusion Inference} \\ \midrule
%         Model & Full Obs.  & Full  & 0.5 & Lim. & minFDE $(\downarrow)$ & minADE $(\downarrow)$  \\ \midrule 
%         K-means PaS~\cite{afolabi2018people}  & \checkmark  & 0.614 & 0.613 & 0.664  & N/A & N/A \\
%         GMM PaS~\cite{itkinaicra2022}  & \checkmark & 0.536 & 0.532 & 0.685 & N/A & N/A \\
%         MAVOI~\cite{itkinaicra2022}  & \checkmark  & 0.614 & 0.613 & 0.664  & N/A & N/A \\\midrule
%         \end{tabular}
%         \label{table:results_v2}
%         \end{center}
% \end{table*} 


==> figures/prediction.tex <==
\begin{figure*}[ht]
\tiny
\centering     %%% not \center
\subfigure[Scene 1: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_3_b-2_False_False.pdf}}
\subfigure[Scene 1: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_3_b-2_False_False.pdf}}
\subfigure[Scene 2: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_47_b-3_False_False.pdf}}
\subfigure[Scene 2: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_47_b-3_False_False.pdf}}

\subfigure[Scene 3: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_289_b-0_False_False.pdf}}
\subfigure[Scene 3: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_289_b-0_False_False.pdf}}
\subfigure[Scene 4: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_291_b-0_False_False.pdf}}
\subfigure[Scene 4: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_291_b-0_False_False.pdf}}

\caption{Scene Informer prediction. We predict both occluded and observed objects represented as black dots. Dotted blue and green lines indicate observation, and ground truth future trajectories, respectively. Anchors are located inside the occlusion polygon (grey) from the perspective of the ego-vehicle (yellow star). Their intensity represents the probability of occupancy. For all scenarios, our approach predicts a high probability of occupancy for the ground truth occluded objects and outputs realistic future trajectories.}
\vspace{-0.3cm}
\label{fig:results}
\end{figure*}


==> figures/visbility.tex <==
% \begin{figure}[h]
% \label{fig:dataset}
% \centering     %%% not \center
% \subfigure[Full]{\label{fig:a}\includegraphics[width=25mm]{figures/full_vis.png}}
% \subfigure[Limited]{\label{fig:b}\includegraphics[width=25mm]{figures/limit_vis.png}}
% \caption{Visualization of the occlusion inference dataset. (Left) Full observability dataset (Right) Limited observability with missing occluded objects from the perspective of the ego-vehicle. Past trajectories and future trajectories are visualized with blue and green colors, respectively. Each data sample contains only single occlusion (grey polygon) from the perspective of the ego vehicle (star). Red dots are anchors which are provided to the decoder. During optimization, we are matching the closest anchor to the to-be-inferred future trajectory.}
% \vspace{-0.3cm}
% \label{fig:dataset}
% \end{figure}

\begin{figure}[ht]
\tiny
\centering     %%% not \center
\subfigure[Full Obs]{\label{fig:a}\includegraphics[width=33mm]{new_figures/2_244_True_567-True_0.35_False_b_0_False_False_v2.pdf}}
\subfigure[Partial Obs (\SI{50}{\percent})]{\label{fig:a}\includegraphics[width=33mm]{new_figures/full_obs.pdf}}
\subfigure[Limited Obs]{\label{fig:b}\includegraphics[width=33mm]{new_figures/limited_obs.pdf}}
\subfigure[Full Obs (Occ. Inf.)]{\label{fig:b}\includegraphics[width=33mm]{new_figures/full_obs.pdf}}
% \subfigure[Scene 3: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_289_b-0_False_False.pdf}}
% \subfigure[Scene 3: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_289_b-0_False_False.pdf}}
% \subfigure[Scene 4: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_291_b-0_False_False.pdf}}
% \subfigure[Scene 4: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_291_b-0_False_False.pdf}}

\caption{Visualization of the occlusion inference dataset. (Left) Full observability dataset (Right) Limited observability with missing occluded objects from the perspective of the ego-vehicle. Past trajectories and future trajectories are visualized with blue and green colors, respectively. Each data sample contains only single occlusion (grey polygon) from the perspective of the ego vehicle (star). Red dots are anchors which are provided to the decoder. During optimization, we are matching the closest anchor to the to-be-inferred future trajectory.}
\vspace{-0.3cm}
\label{fig:results}
\end{figure}


==> new_figures/figures/ablation.tex <==
\renewcommand{\thesubfigure}{}
\begin{figure*}[ht]
\tiny
\centering
\subfigure[Scene 1: Trajectories]{\label{fig:a}\includegraphics[width=36mm]{new_figures/Modified_Ablation_4.pdf}}
\hspace{1cm} % adjust this value to change horizontal spacing
\subfigure[Scene 1: Occupancy]{\label{fig:b}\includegraphics[width=36mm]{new_figures/Modified_Ablation_1.pdf}}
\hspace{1cm} % adjust this value to change horizontal spacing
\subfigure[Scene 2: Trajectories]{\label{fig:a}\includegraphics[width=36mm]{new_figures/Modified_Ablation_3.pdf}}
\hspace{1cm} % adjust this value to change horizontal spacing
\subfigure[Scene 2: Occupancy]{\label{fig:b}\includegraphics[width=36mm]{new_figures/Modified_Ablation_2.pdf}}
\vspace{-0.25cm} % adjust this value to change vertical spacing between rows
\caption{Impact of observed agents' histories on the occlusion inference performance. We modify the observed trajectories of two agents (\bluecircle and \greentriangle). In Scene 1, we visualize a scenario where a \greentriangle\ is stationary and a \bluecircle\ is moving forward. For an anchor \redanchor, our approach predicts occupancy with low probability and vertical motion from the top to the bottom of the intersection. In Scene 2, we visualize the predictions for a modified scenario. The \greentriangle\ is approaching quickly the intersection and the \bluecircle\ is stationary. Scene Informer realistically adapts its occupancy and trajectory predictions based on the observed motion of other agents. It is now highly likely that the anchor in the middle of the occlusion is occupied, and a majority of predicted trajectories are horizontal from the left to right of the intersection.}
\vspace{-0.3cm}
  \label{fig:ablation}
 \end{figure*}
\renewcommand{\thesubfigure}{\alph{subfigure})}
%blue_circle = orange circle

==> new_figures/figures/prediction.tex <==
\begin{figure*}[ht]
\tiny
\centering     %%% not \center
\subfigure[Scene 1: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_3_b-2_False_False.pdf}}
\subfigure[Scene 1: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_3_b-2_False_False.pdf}}
\subfigure[Scene 2: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_47_b-3_False_False.pdf}}
\subfigure[Scene 2: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_47_b-3_False_False.pdf}}

\subfigure[Scene 3: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_289_b-0_False_False.pdf}}
\subfigure[Scene 3: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_289_b-0_False_False.pdf}}
\subfigure[Scene 4: Trajectory]{\label{fig:a}\includegraphics[width=33mm]{figures/pred_traj_291_b-0_False_False.pdf}}
\subfigure[Scene 4: Occupancy]{\label{fig:b}\includegraphics[width=33mm]{figures/pred_occ_291_b-0_False_False.pdf}}

\caption{Scene Informer prediction. We predict both occluded and observed objects represented as black dots. Dotted blue and green lines indicate observation, and ground truth future trajectories, respectively. Anchors are located inside the occlusion polygon (grey) from the perspective of the ego-vehicle (yellow star). Their intensity represents the probability of occupancy. For all scenarios, our approach predicts a high probability of occupancy for the ground truth occluded objects and outputs realistic future trajectories.}
\vspace{-0.3cm}
\label{fig:results}
\end{figure*}

